A first look at the IP eXchange Ecosystem

The IPX Network interconnects about 800 Mobile Network Operators (MNOs) worldwide and a range of other service providers (such as cloud and content providers). It forms the core that enables global data roaming while supporting emerging applications, from VoLTE and video streaming to IoT verticals. This paper presents the first characterization of this, so-far opaque, IPX ecosystem and a first-of-its-kind in-depth analysis of ann IPX Provider (IPX-P). The IPX Network is a private network formed by a small set of tightly interconnected IPX-Ps. We analyze an operational dataset from a large IPX-P that includes BGP data as well as statistics from signaling. We shed light on the structure of the IPX Network as well as on the temporal, structural and geographic features of the IPX traffic. Our results are a first step in understanding the IPX Network at its core, key to fully understand the global mobile Internet.

==> sections/draft_structure.tex <==
% !TeX root = sigcomm19.tex
% ================================================================
\section{Introduction}

\input{introduction}

Short overview of the roaming ecosystem:
\begin{itemize}
\item roaming partners
\item exchange point (roaming hub)
\item clearing house (data and financial clearing)
\end{itemize}

Leverage the real data and operational realities we collect from a consortium of mobile operators (start with Telefonica and expand to other potential partners from there). 

Datasets we use/need: 
\begin{itemize}
\item interaction with third parties specialized in data and financial clearing
\item characteristics of the roaming agreements and how operators express preferences between roaming partners
\item actual CDR information to present the roaming trends on different timescales
\item interaction with roaming hubs (IPX) 
\end{itemize}

\section{Mobile Roaming Background}

% give a basic definition of what roaming is, how people use it and how regulation impacted it
% this is the background section together with Related work  
% not obvious about the overlap with the section below -- I think it might be better to just merge these

Discuss both national and international roaming. 

Interleave the information above with the different radio access technologies (focus on 3G and 4G) and the different types of traffic.

Discuss the infrastructure operators and the MVNOs as well. 


\section{The Roaming Ecosystem}

% should describe here the different solutions for roaming
% should look into interaction with the roaming hub 
% introduce the clearing house and describe the interaction between roaming partners 

\section{The Roaming Business}

% bring into play the business aspects of roaming 
% talk about the need for a roaming hub, and its interaction with bilateral agreements 

\section{The Anatomy of an IPX Provider}
% describe how MNOs are actually implementing roaming 
% talk about the shortcoming of the current solutions, describe current structural (regulation) and technical barriers 
% back this up with data from networks 
% for example, we can look at roaming in LATAM vs. roaming in EU 

\section{Roaming Trends: view from an MNO}
% depending on the data we get from Telefonica and other networks 
% we can look at the patterns of inbound and outbound roamers from the perspective of mobile users
% correlate this with flight information? 

% analysis of anomalies in the IPX 

\section{Roaming in Future Mobile Networks}
% VoLTE, 5G 

==> sections/introduction-feb.tex <==
% !TeX root = sigcomm20.tex
% ================================================================

\section{Introduction}
\label{sec:introduction}

Traditionally, the interconnection between Mobile Network Operators (MNO) for international roaming has been achieved through bilateral agreements, where two MNOs in different countries established a roaming agreement and set the correspondent interconnection. While this model was sufficient when roaming was a niche service, affordable to large MNOs that generated a marginal amount of traffic, it has proven to be insufficient in recent years.

Today's demand on international roaming and a shift to all-IP-based services have brought new impetus to the old idea of \ac{IPX}. The \ac{IPX} interconnection model was first proposed by \ac{GSMA} back in 2007 for the exchange of IP-based traffic between customers of mobile and fixed operators and other types of service provider (e.g., ISPs, IoT providers, Online Service providers). Under the IPX model, \acp{IPX-P} offer roaming and interconnection services
to MNOs and other Service Providers (SPs), and connect to other IPX-Ps to expand their coverage. The resulting IPX Network is an isolated network that bypases the public Internet~\cite{manynet}, to ensure secure, SLA-compliant services, from video streaming and AR/VR to VoIP and IoT verticals, such as connected cars.

Due in part to this intrinsic opacity, no previous work has analyzed the IPX Network or its associated ecosystem. In this paper, we present the first characterization of the IPX ecosystem and a first-of-its-kind, detailed study of a large IPX provider.

International roaming is becoming increasingly common fueled both by the number of international travelers, reaching 1.4 billion in 2018,\footnote{\url{https://www.e-unwto.org/doi/pdf/10.18111/9789284421152}} and the 
reduction/elimination of roaming fees in large geographical areas~\cite{}. International roaming 
services have now become a commodity available across all mobile providers, including small and even virtual providers~\cite{}.

To satisfy user expectations for quality of experience -- when using VoIP, accessing maps or posting pictures -- content and service providers need connections close to their users, wherever they are roaming. This means connecting as directly as possible to all MNOs providing roaming services, thus becoming part of the interconnection ecosystem.

In addition to people roaming, the support of ``things'' that roam internationally have become critical for vertical applications in the \ac{IoT} space, from wearables to connected cars and logistics. This results both from the re-purposing of MNOs' infrastructures to support \ac{IoT} and \ac{M2M} services and the adoption of a model for \ac{IoT} connectivity where international shipped devices come with pre-arranged connectivity at the original provider's original location.\footnote{In contrast to a model where IoT providers make local arrangements in the country where devices are used to obtain connectivity.}

\enote{FEB}{The contributions should probably need to be done in paragraphs rather than bullet points; that would mean including a contribution, explanation, highlighted observations, ref to the section that correspond.}

\enote{ael}{start building the list of contributions}
The contributions we bring in this paper are as follows:
\begin{itemize}
\item A complete characterization of interconnectivity in the cellular ecosystem, with a focus on the roaming requirements. 
\item A first look at the anatomy of an IPX Provider and the characterization of the IPX Network using data from an IPX Service provider (via Telefonica Global solutions) 
%and also from a Mobile Network operator connecting to the IPX Network (via data from an MNO in UK). %\ael{the view from the MNO can be a separate contribution on itself}
%\item Using the previous results, we build an anomaly detection method able to alert the IPX Provider of irregularities/deviations. The alarm triggering system enables the IPX providers to take proactive mitigation approaches.
%\ael{this last point may as well be just an analysis of anomalies within an IPX provider; or we can just drop this last point if you think it does not really fit here}
\end{itemize}

==> sections/introduction-marcelo.tex <==
% !TeX root = sigcomm20.tex
% ================================================================

\section{Introduction}
\label{sec:introduction}

In this paper, we present the first characterization of the IPX ecosystem and a first-of-its-kind, detailed study of a
large \acp{IPX-P}. Due in part to this intrinsic opacity, no previous work has analyzed the IPX Network or its associated ecosystem. 

Traditionally, the interconnection between \ac{MNO} for international roaming has been achieved
through bilateral agreements, where two \acp{MNO} in different countries established a roaming agreement and set the
correspondent interconnection. While this model was sufficient when roaming was a niche service, affordable to large
MNOs that generated a marginal amount of traffic, it has proven to be insufficient in recent years. Over the last decade, 
the scalability of the roaming ecosystem has been stressed by the addition of numerous  new players.

International roaming is becoming increasingly common fueled both by the number of international travelers, 
reaching 1.4 billion travellers in 2018,\footnote{\url{https://www.e-unwto.org/doi/pdf/10.18111/9789284421152}} and
the reduction/elimination of roaming fees in large geographical areas~\cite{}. International roaming 
services have now become a commodity available across all mobile providers, including small and even virtual 
providers~\cite{}.

To satisfy user expectations for quality of experience -- e.g. when using VoIP, accessing maps or posting pictures -- 
content and other service providers need connections close to their users, wherever they are roaming. This means 
connecting as directly as possible to all MNOs providing roaming services, thus becoming also part of the 
roaming interconnection ecosystem.

In addition to people roaming, the support of ``things'' that roam internationally have become common for 
vertical applications in the \ac{IoT} space, from wearables to connected cars and logistics. This results both 
from the re-purposing of MNOs' infrastructures to support \ac{IoT} and \ac{M2M} services and the adoption of a 
model for \ac{IoT} connectivity where international shipped devices come with pre-arranged connectivity at the 
original provider's original location.\footnote{In contrast to a model where IoT providers make local arrangements 
in the country where devices are used to obtain connectivity.}

Today's demand on international roaming and a shift to all-IP-based services have brought new impetus to the old 
idea of \ac{IPX}, proposed by \ac{GSMA} back in 2007. The IPX Network serves as a hub for international roaming
services and it is the network resulting from the interconnection of multiple \ac{(IPX-Ps}. IPX-Ps offer global
interconnection services between mobile and fixed operators and other types of service provider (e.g., ISPs,  IoT
providers, Online Service providers) across the globe for the purposes of international roaming. They offer a global,
private, secure, IP network service with end-to-end Quality of Service (QoS), service aware gateways (known as IPX
proxies) to manage IP based application service exchanges, and cascading interconnect payments. 


\enote{FEB}{The contributions should probably need to be done in paragraphs rather than bullet points; that would mean
	including a contribution, explanation, highlighted observations, ref to the section that correspond.}

\enote{ael}{start building the list of contributions}
The contributions we bring in this paper are as follows:
\begin{itemize}
	\item A complete characterization of interconnectivity in the cellular ecosystem, with a focus on the roaming
	requirements. 
	\item A first look at the anatomy of an IPX Provider and the characterization of the IPX Network using data from an IPX
	Service provider (via Telefonica Global solutions) 
	%and also from a Mobile Network operator connecting to the IPX Network (via data from an MNO in UK). %\ael{the view
	%from the MNO can be a separate contribution on itself}
	%\item Using the previous results, we build an anomaly detection method able to alert the IPX Provider of
	%irregularities/deviations. The alarm triggering system enables the IPX providers to take proactive mitigation
	%approaches.
	%\ael{this last point may as well be just an analysis of anomalies within an IPX provider; or we can just drop this
	%last point if you think it does not really fit here}
\end{itemize}



==> sections/ipx_mobility.tex <==
% !TeX root = sigcomm20.tex
% ================================================================
%section 2 --> what is IPX
%section 3 --> who uses IPX
%section 4 --> example of one operational IPX-P
%section 5 --> how are customers using the signaling platforms of the IPX-P
%section 6 --> how are customers using the data platform of the IPX-P

\begin{figure}[tb!]
	\includegraphics[width=.98\columnwidth]{./figures/figs_signaling/mobility_matrix_allSignaling_20191201-14.png}
	%\vspace{-4mm}
	\caption{\small Mobility dynamics based on SCCP global signaling data (devices using 2G/3G) and Diameter signaling
		data (devices using 4G/LTE).}
	\label{fig:roaming_dynamics}
	\vspace{-6mm}
\end{figure}

%We focus on the countries where this IPX-P has customers and capture the mobility 
%		patterns of devices between operators in these countries.

\section{Mobility Analysis}
\label{sec:mobility}

Having analyzed the signaling and data roaming services of the IPX-P, in the next paragraphs we focus on how 
MNO subscribers use the IPX platform for roaming, their mobility patterns and data communication usage. 
%We first rely on the signaling dataset to look at their mobility and then use the data roaming dataset to analyze
%the performance of the roaming platform  finding that most tend to have a handful of 
%preferred roaming countries. 


%For example, we find that 71\% of all devices from Venezuela using this IPX-P in December 2019 travel to Colombia.

%****************************************
\subsection{Mobility Patterns} 

We rely on the signaling dataset to characterize the (international) mobility of devices. Figure~\ref{fig:roaming_dynamics} 
shows the distribution of mobile devices, registered during the observation period (1-14 December 2019), that travel from their home 
country (column) to a visited country (row). Overall, we find that the majority of subscribers using the IPX-P 
infrastructure - serving large European MNOs -- comes from UK ($\approx$8 million devices in December 2019), 
Germany ($\approx$2 million devices) or Spain ($\approx$2 million devices). Most of these devices
tend to visit the UK ($\approx$6.5 million devices), Germany ($\approx$2.5 million devices) or the US ($\approx$500,000 devices). 

\textit{When clustered by geographic regions (i.e, Europe and the Americas), we see that the most popular destinations roamers 
visit include the UK in Europe and the US in America.} Indeed, Figure~\ref{fig:roaming_dynamics} shows that the UK 
operators connected to the IPX-P we analyze receive 34\% of all the devices from Germany (DE) visible in the system, 85\% 
of the devices from the Netherlands (NL), and 45\% of all devices from Spain (ES), among others. Interestingly, we verified with 
the British operator connected to our IPX-P and found that the inbound roaming devices from the Netherlands ($\approx$~7.8 million devices) are \ac{IoT} 
devices deployed by energy providers (smart meters)\footnote{This is consistent with deployment of the Smart Metering 
Implementation Programme of the U.K. government. In 2019, there were 15.4 million smart meters deployed in the UK~\cite{smartmeter}.}.
US, Brazil and Mexico emerge as the most popular destinations in the Americas.
Specifically, the US operators connected to our IPX-P accommodate 79\% of all the outbound roaming devices from Mexico (MX)
using the IPX-P infrastructure, 44\% of all outbound roaming devices from El Salvador (SV), 17\% of all outbound roaming
devices from Colombia (CO) and 22\% of all outbound roaming devices from Brazil (BR). 
\textit{We also note the impact of the migration between Venezuela and Colombia, with 71\% of the subscribes from Venezuela (VE)
traveling to Colombia (CO) during the period we capture. Inversely, we find that 56\% of all Colombian outbound roamers
travel to Venezuela (VE). 
}

%We further scope our analysis here to only capture the mobility within the above-mentioned countries in Latin America. 
%This represents a total of $\approx$2 million mobile devices. 
%The three countries with the highest population of outbound data roamers are Colombia, Venezuela and Brazil. 
%This distribution is specific to the vantage point we use in order to capture the international mobility of roamers. 
%Figure~\ref{fig:roaming_dynamics} shows the percentage of devices that we register in our system during the first two
%weeks of December 2019 that travel from their home country (column) to a visited country (row).

%****************************************
\subsection{Steering of Roaming}

\begin{figure}[tb!]
	\centering
	\includegraphics[width=\linewidth]{figures/figs_signaling/steering_of_roaming.png}%
	\caption{\small Steering of Roaming Service Analysis: Percentage of devices that travel from home country to visited
		country for which the IPX-P triggered \textit{Roaming Not Allowed} at least once over a period of two weeks in December
		2019. }
	\label{fig:steering_of_roaming}
	\vspace{-3mm}
\end{figure}

By using \textit{Steering of Roaming (SoR)} an MNO can specify the preferred roaming partner in a given visited country and allow
the IPX-P to enforce those preferences. With this in place, if a roamer device traveling outside its home network (HMNO)\footnote{An MNO can 
use the IPX-P within the same home country for national roaming or for enabling virtual operators, as well as in foreign
countries for international roaming.} attempts to attach to a less preferred roaming partner, the IPX-P will force
the \textit{Roaming Not Allowed} response code (RNA, error code = 8) to an \ac{UL} message intercepted from the visited 
network (VMNO). The IPX-P will then try steering the roamer to one of the HMNO's preferred roaming partners after forcing four UL 
attempts from the roamer to fail, unless no preferred roaming partner is available in the area (in which case, the SoR platform 
triggers an exit control to avoid the risk of the roamer not receiving service at all). 

% The IPX-P will try steering the roamer to a HMNO's preferred roaming partner at most four times before giving up (e.g., because there is no preferred roaming partner in the area). 

Figure~\ref{fig:steering_of_roaming} shows the percentage of end-user devices roaming from the home country
(column-wise) to a visited country (row-wise) for which we registered at least one RNA
error code for the \ac{UL} procedure. \textit{We observe a non-negligible number of \textit{Roaming Not Allowed} operational
code as a result of the \ac{UL} request from the VMNO, typically due to the use of the SoR service the IPX-P provides 
its customers.}

One notable exception is Venezuela. We note the prevalence of this error code for mobile subscribers traveling from 
Venezuela abroad, regardless the visited country. Because of the volatility of Venezuelan currency, mobile operators in 
Venezuela suspended international roaming as they said they lacked enough foreign currency to pay roaming partners in foreign 
countries. The reason this is allowed for Spain (where we only note that 20\% of subscribers from Venezuela receive a RNA 
message) is because of internal agreements between operators that belong to the same international corporation. 

On the other end of the spectrum, we see that the fraction of UK users (marked GB in Fig.~\ref{fig:steering_of_roaming}) 
affected by this error code is very small, regardless of the country they visit. This is because the
IPX-P's customer in the UK does not use the SoR service from the IPX-P, but instead handles the steering of its
subscribers separately. Thus, the RNA errors we capture are due to the HMNO from UK not allowing its subscribers to roam
(e.g., because of billing issues, etc.).
%This is because the IPX-P implements a different procedure for the Steering of Roaming service, specific only for their
%UK customer. 
%Here, the IPX-P does not intercept the UL messages (which reach the home network), but instead blocks sending the
%Subscriber Data to the less optimal visited network, forcing the latter to drop the mobile subscriber. 


% \ael{cite https://en.wikipedia.org/wiki/Venezuelan_bol\%C3\%ADvar}


%****************************************
\subsection{Silent Roamers}

Despite the dynamic global movement of mobile subscribers, not all might be active in terms of data communications.
Data communications while roaming have often generated bill shock for mobile subscribers or kept roamers silent (i.e.,
they do not trigger data communications).
%\footnote{https://www.nytimes.com/2019/10/26/world/europe/eagles-data-roaming-charges.html} 
Thus, when traveling to a foreign country, mobile subscribers often turn off the data communication capabilities of
their devices to avoid high bills.
Even if this may no longer be the case for roamers inside Europe~\cite{lh_regulation}, we find that majority of roamers
within Latin America are still silent. 

%Thus, we focus our analysis on roamers between Latin American countries where the IPX-P has customers with significant
%volume of subscribers (Brazil, Argentina, Colombia, Costa Rica, Ecuador, Peru and Uruguay).
By contrasting the mobility of users from signaling dataset (regardless the radio access technology) with the activity we
register in the data roaming dataset (active GTP tunnels, see Section~\ref{sec:signaling_analysis}), we are able to quantify the amount of silent roamers. 
For the first two weeks of December 2019, we capture the signaling activity of $\approx$ 2 million subscribers roaming between the 
Latin American countries where the IPX-P has significant volume of subscribers 
(Brazil, Argentina, Colombia, Costa Rica, Ecuador, Peru and Uruguay).
Out of these, we find that $\approx$400,000 mobile devices only are using data services while traveling abroad within
Latin America.
For these, we observe in Figure~\ref{fig:roaming_data} that the amount of total traffic volume per session (uplink or
downlink) is no more than 100KB, in average, per device.
% This represents 60\% of all the devices active abroad within Latin America according to the signaling dataset. 

Even more, when focusing on \textit{inbound} roamers in Latin America (regardless the home country), we also capture $\approx$2,5 million IoT devices
provisioned by one of the IPX-P's M2M customers.
The latter provisioned the IoT devices operating in Latin America with connectivity from a Spanish MNO. 
We compare the amount of traffic each roamer within Latin America generates with the amount of traffic from IoT devices
(Figure~\ref{fig:roaming_data}).
\textit{We find that, although "things" generate very little traffic in general, mobile subscribers within Latin America have a
very similar behavior (though tend to transfer slightly larger data volumes than that from IoT devices).
We conjecture this is the result of the lack of regulation on roaming within the region, as well as the socio-economic
landscape, which keep the cost of roaming data communications prohibitive.}
%The latter are well-know to rely on signaling activity mostly and only trigger occasional and seldom data
%communications. 

==> sections/ipx_performance.tex <==
% !TeX root = sigcomm20.tex
% ================================================================

\section{Data Roaming Analysis}
\label{sec:performance}

In this section, we explore the data roaming dataset (see Table~\ref{table:datasets}) and give further insights into the type of traffic flowing through the IPX Network and its performance.  
The IPX-P we study deploys a mediation platform for monitoring that centralizes large amounts of data from the different network elements that are part of the infrastructure they operate. 
The mediation platform receives and processes raw data to generate statistics in real time for the traffic flowing on the Gn interface between the SGSN and GGSN nodes that are part of the GPRS core network (2G/3G) or the S11 or S5/S8 interfaces between the SGw and the PGw in case the EPC is used (4G/LTE). 
These are packet interfaces for sending IP traffic uplink or downlink to the mobile terminal. 
%The IPX-P uses \ac{GTP} for setting up and tearing down tunnels between the above-mentioned nodes for user data across the IPX Network.
Specifically, the mediation platform captures on the traffic that terminates or originates at mobile subscribers that belong to the IPX-P's customers in Latin America, as well as to its \ac{M2M} customers. 
Our data roaming dataset represents a two-weeks-long snapshot of the traffic statistics from the mediation platform. 


\subsection{Data Roaming Mobility}

Data communications while roaming have often generated bill shock for mobile subscribers.\footnote{https://www.nytimes.com/2019/10/26/world/europe/eagles-data-roaming-charges.html} 
Thus, when traveling to a foreign country, mobile subscribers often turn off the data communication capabilities of their devices to avoid high bills.
Even if this may no longer be the case for roamers inside Europe~\cite{lh_regulation}, we find that majority of roamers within Latin America are still silent (i.e., they do not trigger data communications). 
For this analysis, we focus on roamers between Latin American countries where the IPX-P has customers with significant volume of subscribers (Brazil, Argentina, Colombia, Costa Rica, Ecuador, Peru and Uruguay).
% By contrasting the mobility of users from signaling data (Section~ref{sec:signaling_analysis}) with the activity we register in the data roaming dataset, we are able to quantify the amount of silent roamers. 

\begin{figure}[tbh]
  \includegraphics[width=.98\columnwidth]{./figures/figs_signaling/mobility_allSignalling_latam_only.png}
    %\vspace{-4mm}
  \caption{\small Mobility dynamics based on SCCP global signaling data (devices using 2G/3G) and Diameter signaling data (devices using 4G/LTE). 
  We target here only the countries where this IPX-P has customers and capture the roaming of devices between operators in these countries ($\approx$2 million subscribers)  
  For example, we find that 71\% of all devices from Venezuela using this IPX-P in December 2019 travel to Colombia.}
  \label{fig:roaming_dynamics}
  \vspace{-6mm}
\end{figure}

We first investigate the mobility dynamics of roaming mobile subscribers strictly from signaling data, as seen from the IPX-P we analyze.
This shows us the presence of subscribers in a visited country (i.e., that they attached to the radio network of a local VMNO). 
Overall, we find that, given that the IPX-P serves large customers in Europe, the majority of subscribers using the IPX-P's infrastructure comes from UK ($\approx$8 million devices), Germany ($\approx$2 million devices) or Spain ($\approx$2million devices).
Similarly, most devices visit UK ($\approx$6.5 million devices), Germany ($\approx$2.5 million devices) or US ($\approx$500,000 devices). 
We scope our analysis here to only capture the mobility within the above-mentioned countries in Latin America. 
This represents a total of $\approx$2 million mobile devices. 
The three countries with the highest population of outbound data roamers are Colombia, Venezuela and Brazil. 
This distribution is specific to the vantage point we use in order to capture the international mobility of roamers. 
Figure~\ref{fig:roaming_dynamics} shows the percentage of devices that we register in our system during the first two weeks of December 2019 that travel from their home country (column) to a visited country (row).
We note the impact of the migration between Argentina and Colombia, with 86\% of the subscribes from Argentina traveling to Colombia during the period we capture. Inversely, we find that 60\% of all Colombian outbound roamers travel to Venezuela. 
 

%In terms of visited countries, the most popular destinations include the UK in Europe and the US in America. 
%Indeed, Figure~\ref{fig:roaming_dynamics} shows that the UK operators connected to the IPX-P we analyze receive 44\% of all the devices from Germany that use the IPX-P's infrastructure, 87\% of the devices from the Netherlands, and 32\% of all devices from Spain, among others.  
%Interestingly, we verified with the British operator connected to our IPX-P and found that the inbound roaming devices from the Netherlands are \ac{IoT} devices deployed by energy providers (smart meters).
%In Latin America, Brazil and Mexico seem to be the most popular destinations.
%Specifically, the US operators connected to our IPX-P accommodate 88\% of all the outbound roaming devices from Mexico using the IPX-P infrastructure, 45\% of all outbound roaming devices from El Salvador, 37\% of all outbound roaming devices from Peru and 33\% of all outbound roaming devices from Brazil. 
%Thus, the UK and the US are the two most important mobility hubs for the two regions that our IPX-P covers. 

Despite this dynamic movement of mobile subscribers, we find that only a small fraction is active in terms of data communications. 
In the data roaming dataset, we capture (from the user plane) the Create/Delete \ac{PDP} context procedures that the devices triggers before/after a data communication. 
Specifically, the mediation platform generates one record for the Create Session Request/Response exchange and retains basic information, such as the tunnel ID. 
Then, the mediation platform generates a final record when the session is deleted, which captures statistics for the whole session, such as the total amount of bytes transferred. 
%This allows us to quantify the amount of mobile subscribers which 
Overall, we find that $\approx$1.2 million mobile devices only are using data services while traveling abroad within Latin America (namely, Brazil, Argentina, Colombia, Costa Rica, Ecuador, Peru and Uruguay).
This represents 60\% of all the devices active abroad within Latin America according to the signaling dataset. 

Even more, when focusing on inbound roamers in Latin America, we find $\approx$2,5 million devices provisioned by one of the IPX-P's M2M customers.
We compare the amount of traffic each smartphone consumes with the amount of traffic from IoT devices.
We find that, although "things" generate very little traffic in general, in our particular case the amount of bytes transferred on average by smartphones is also very small, though slightly larger than that from IoT devices.  

%\ael{include here the comparison between the amount of data traffic -- the CDFs}
 
%\begin{figure}[t!]
%	\centering	
%	\begin{subfigure}{0.45\columnwidth}
%		\includegraphics[width=\linewidth]{figures/figs_data/ip_heatmap_latam_outbound_1201}%
%		\caption{Outbound.}%
%		\label{fig:ip_outbound}%
%	\end{subfigure}%
%	\begin{subfigure}{0.45\columnwidth}
%		\includegraphics[width=\linewidth]{figures/figs_data/ip_heatmap_latam_inbound_column_1201.png}%
%		\caption{Inbound.}%
%		\label{fig:ip_inbound}%
%	\end{subfigure}%	
%	\caption{\small Mobility of mobile subscribers with at least one data session during their roaming session. We show the subscribers traveling outbound (a) and inbound (b) from Latin America (column-wise, the countries where the IPX-P has clients) to and from, respectively, the top most popular visited countries (row-wise). We aggregate the values column-wise (i.e., on a column, values should sum to 100\%). }
%	\vspace{-3mm}
%\end{figure} 
 
%Figure~\ref{fig:ip_outbound} shows the breakdown of outbound roamers from the Latin American countries where the IPX-P has customers with significant volume of subscribers (namely, Brazil, Argentina, Colombia, Costa Rica, Ecuador, Peru and Uruguay) to the most popular visited countries worldwide. (i.e., where more than 3\% of the outbound roamers travel). 
%We note, for example, that 23\% of the subscribers from Argentina travel to Brazil, 18\% to Chile and 15\% to the US. 
%Overall, we note that US represents a popular visited country, where large fractions of the mobile subscribers we capture in the dataset travel (e.g., 19\% of subscribers from Brazil, 37\% from Colombia, 34\% from Ecuador or 23\% from Peru).
%Similarly, Brazil is also a popular destination, attracting a large number of the mobile subscribers we capture in our dataset. 
%We observe the difference with the distribution we capture from the signaling traffic in Figure~\ref{fig:roaming_dynamics}. 
%The latter integrates the "silent" roamers, who do not trigger data communications while roaming internationally and, thus, do not generate any revenue for the visited \ac{MNO}.

\subsection{Roaming Traffic Breakdown}

\begin{figure}[thb!]
	\centering
	
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=\linewidth]{figures/figs_data/ip_protocols_1201.png}%
		\caption{Total traffic breakdown.}%
		\label{fig:application_traffic}%
	\end{subfigure}%	
	
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[width=\linewidth]{figures/figs_data/ip_protocols_tcp_1201.png}%
		\caption{TCP traffic breakdown.}%
		\label{fig:tcp_traffic}%
	\end{subfigure}%
	
    \begin{subfigure}{0.5\textwidth}
		\includegraphics[width=\linewidth]{figures/figs_data/ip_protocols_udp_1201.png}%
		\caption{UDP traffic breakdown.}%
		\label{fig:udp_traffic}%
	\end{subfigure}%
	
	\caption{\small Data traffic mix for all data roaming we capture during 1-14 Dec. 2019. }
	\vspace{-3mm}
\end{figure} 
 
On the user plane, each data record captures different applications that correspond to the subscriber activity over the period we monitor (1-14 December 2019), including WAP, MMS, SMTP, RTP, IP, TCP, UDP, FTP.  
The data record integrates performance parameters per roaming data communication, including \ac{RTT}, packet retransmissions or volume of bytes transferred (uplink and downlink). 
Figure~\ref{fig:application_traffic} shows the breakdown of the mix of traffic we capture in the data roaming dataset.
We note that the majority of the traffic is TCP or UDP, but we also capture application-specific traffic, such as WAP, FTP or MMS. 
The destination port breakdown for the TCP records we capture in the user plane (Figure~\ref{fig:tcp_traffic}) reveals that the largest amount of traffic is web traffic (HTTP, HTTPS).
The breakdown UDP traffic in Figure~\ref{fig:udp_traffic} shows that majority is DNS traffic. 
This is (largely) due to the procedure the \acp{MNO} roaming partners implement in order to allow for international context creation (tunnels) over the IPX Network (i.e., control traffic).
The \ac{VMNO} uses the IPX to resolve the \ac{APN} associated to the mobile subscriber to an actual IP address corresponding to the home network \ac{GGSN} (or PGw for EPC), which the \ac{HMNO} performs.
 
For the web browsing traffic, we further check the \ac{RTT} distribution the mobile subscribers experiment, broken down per visited country. 
We note that, because of the home routed roaming configuration (Figure~\ref{fig:roaming_type}), the RTT varies with the distance between the home country (in this case, Brazil) and the visited country. 




==> sections/ipx_sig_traffic.tex <==
% !TeX root = sigcomm20.tex
% ================================================================

\begin{figure}[th!]
	\centering
	
	\begin{subfigure}{0.95\columnwidth}
		\includegraphics[width=\linewidth]{figures/figs_signaling/sig_records_sum_MAP_diameter_201911.png}%
		\caption{\tiny Signaling traffic volume and number of devices active in each platform (SCCP Signaling and Diameter
			Signaling).}%
		\label{fig:signaling_time_series_all}%
	\end{subfigure}%
	
	\begin{subfigure}{0.95\columnwidth}
		\includegraphics[width=\linewidth]{figures/figs_signaling/map_records_agg_per_hour_201912.png}%
		\caption{\tiny SCCP signaling traffic breakdown per type of procedure.}%
		\label{fig:signaling_time_series_MAP}%
	\end{subfigure}%
	
	\begin{subfigure}{0.95\columnwidth}
		\includegraphics[width=\linewidth]{figures/figs_signaling/sig_records_average_per_hour_201912.png}%
		\caption{\tiny Average and standard deviation of the number of SCCP messages and Diameter messages per IMSI per hour.}%
		\label{fig:signaling_avg_time_series}%
	\end{subfigure}%	
	
	\caption{\small Signaling traffic time series for the observation period of December 2019.}
	\label{fig:signaling_time_series}
	\vspace{-3mm}
\end{figure}

%********************************************************************************
\section{System Analysis}
\label{sec:signaling_analysis}
In this section, we provide insights into the complexity of the operations of the IPX-P by analyzing the main services it provides. First, we focus on the radio signaling services -- SCCP Global Signaling and LTE Diameter -- that are mandatory for the correct operation of data roaming and any other IPX-P service. We also look at the impact of an M2M platform operating on the top of the IPX-P signalling infrastructure.
%In this section, we analyze radio signaling in the context of the IPX-P, and provide insights into the complexity of its operations.
Second, we capture dynamics of data roaming, focusing on the GTP tunnels the IPX-P creates between roaming partners to enable data communications for the mobile subscriber. 

%The SCCP Global Signaling and LTE Diameter datasets we collect from the IPX
%comprise signaling information for 2G/3G and 4G/LTE radio technologies from all the devices that use the IPX-P's
%infrastructure (see Table~\ref{table:datasets}, Figure~\ref{fig:diameter_signaling}).

%\enote{DP}{If we split the following paragraph can go with the previous section}
%Overall, the total number of IMSIs we capture over the period we show in Figure~\ref{fig:signaling_time_series} is of
%more than 130M active in 2G/3G and more than 15M active in 4G/LTE\footnote{Note that there might be an overlap between
%these two sets. However, we aim to show here the load on the two different signaling infrastructures.}
%They correspond to 215 home countries and 210 visited countries. 
%The IPX-P's customer are active within 19 countries and include \acp{MNO}, IoT/M2M connectivity providers and cloud
%service providers. 

%****************************************
\subsection{Signaling Traffic Trends}

Figure~\ref{fig:signaling_time_series} shows signaling activity of roaming mobile subscribers during the 
observation period of December 2019. We look at both \ac{MAP} and Diameter signaling procedures. \ac{MAP} is the most 
important application protocol in the \ac{SS7} stack, and handles the roamers' mobility between countries. Although 
this is still the most used protocol for mobile interconnection application messages, the use of the more recent 
Diameter~\cite{rfc6733} signaling protocol has been growing with the adoption of LTE.

Figure~\ref{fig:signaling_time_series_all} focuses on the total signaling traffic and on the number of different 
mobile subscriber devices that generate this traffic. 

\textit{We find that the number of devices using 2G/3G infrastructure 
(extracted from MAP traffic) is an order of magnitude higher than those using 4G infrastructure (based on the Diameter 
traffic). The volume of signaling traffic in the SCCP infrastructure is, correspondingly, more significant in terms 
of total volume than in the Diameter infrastructure.} 
We also note the typical daily and weekly traffic patterns on mobile subscribers' activities. For instance, December 1st was a Sunday, showing the expected decreasing trend in signaling traffic activity which can be seen again the following weekend (December 7-8th). 

Each record in this dataset represents a signaling procedure that a network element triggers, corresponding to different
standard routines. For instance, from the \ac{MAP} interface we capture mobility management routines, including 
location management and authentication. Figure~\ref{fig:signaling_time_series_MAP} shows the time series of signaling 
traffic broken down by type of signaling procedure, including Update Location (UL), Cancel Location (CL) and Send Authentication Information (SAI) messages. The latter, SAI, represents the highest fraction of MAP signaling traffic. Indeed, 
according to the GSM standard definition, the \ac{SGSN} in the visited network triggers the authentication of subscriber 
procedure upon IMSI attach, location update or before starting data communication, thus explaining the larger volume of SAI messages. 

% \ael{cite https://www.etsi.org/deliver/etsi_tr/123900_123999/123909/03.00.00_60/tr_123909v030000p.pdf}, 

Figure~\ref{fig:signaling_avg_time_series} shows the average number of records per IMSI calculated over all the IMSIs we
observe in each one-hour interval (continuous line) during the observation period, as well as the standard
deviation of the number of records per IMSI calculated over all the IMSIs active in the same one hour interval (shaded
area). We observe both the MAP procedures for 2G/3G (red color) and the similar Diameter procedures for 4G/LTE (green color). 
%Even if Diameter is a different protocol than MAP, the underlying functional requirements (e.g., authenticating the
%user to set up a data communication) have many similarities in terms of the messages used for Diameter and the SS7 MAP
%protocol messages. 
%Still, there is not a one-to-one mapping between MAP and Diameter messages. We note that the load in terms of average
%signaling records per IMSI is in the same order of magnitude (the continuous lines on the plot) regardless the radio
%technology and the infrastructure the devices use. 
%However, there are significantly more messages for MAP, as the MAP procedures are more than Diameter
%procedures~\cite{rfc6733, rfc7075} .
While Diameter and MAP are different protocols, the underlying functional requirements (e.g.,
authenticating the user to set up a data communication) have many similarities in terms of the messages used for
Diameter and the SS7 MAP protocol implementation. We note that the load in terms of average signaling records per IMSI is in
the same order of magnitude (the continuous lines on the plot), regardless of the infrastructure the devices use; yet, 
there are significantly more messages for MAP, as Diameter is a more efficient protocol than MAP~\cite{rfc6733, rfc7075}.
%as the MAP procedures are "chattier" than Diameter ones~\cite{rfc6733, rfc7075}.

\begin{figure}[tb!]
	\centering
	\begin{subfigure}{0.5\columnwidth}
		\includegraphics[width=\linewidth]{figures/figs_signaling/map_stp_dist.png}%
		\caption{\tiny  SCCP global signaling.}%
		\label{fig:sig_load_map}%
	\end{subfigure}%
	\begin{subfigure}{0.5\columnwidth}
		\includegraphics[width=\linewidth]{figures/figs_signaling/ngn_dra_dist.png}%
		\caption{\tiny Diameter signaling.}%
		\label{fig:sig_load_diameter}%
	\end{subfigure}%
	\caption{\small Signaling traffic load (total number of records) per infrastructure element per day for SCCP platform
		and Diameter. The boxplots capture the first two weeks in December 2019. }
	\label{fig:sig_load_infrastructure}
	\vspace{-3mm}
\end{figure}

We further investigate the traffic load on the signaling infrastructure, both for the SCCP (with \acp{STP} in Frankfurt,
Madrid, Miami and Puerto Rico) and the Diameter signaling infrastructure (using \acp{DRA} in Frankfurt, Madrid, Miami
and Boca Raton). 
Figure~\ref{fig:sig_load_infrastructure} shows the aggregated signaling traffic (number of messages) per infrastructure
point per day over the same observation period. We note that the redundant deployment of infrastructure
points in each geographical area allows the IPX-P to load-balance the signaling traffic across them (e.g., for 4G
between Frankfurt and Madrid in Europe and between Miami and Boca Raton in America). Signaling traffic in Europe through
the signaling points in Frankfurt and Madrid is considerably higher than that flowing through the signaling points in
America (Miami and Boca Raton/Puerto Rico). This is true for both the SCCP infrastructure
(Fig.~\ref{fig:sig_load_map}) and the Diameter infrastructure (Fig.~\ref{fig:sig_load_diameter}). When comparing the
two signaling services (i.e., SSCP and Diameter), we also note that the traffic volume in the SCCP signaling
infrastructure is approximately twice larger than the traffic volume flowing through the Diameter signaling
infrastructure. This proves the continued popularity of 2G/3G services in the region served by the IPX-P. 

%****************************************
\subsection{Impact of IoT Devices}

The previous analysis does not distinguish between device types (i.e., smartphones or IoT devices). In the
following paragraphs we focus on the traffic corresponding to the IoT devices that the IPX-P M2M platform
operates. 

% those of signaling traffic for M2M devices with statistics 
Figure~\ref{fig:m2m_signaling} shows the time series of average number of signaling messages per device for 2G/3G
(Fig.~\ref{fig:signaling_m2m_map}) and 4G/LTE (Fig.~\ref{fig:signaling_m2m_diameter}), as well as the 95th
percentile calculated over one hour intervals. To put this figures in context, we include statistics from a similar 
number of smartphones using the same radio technology. We selected the set of smartphones leveraging the device 
brand information, which we retrieve by checking the \ac{IMEI} and the corresponding \ac{TAC} code, and included 
only iPhone and Samsung Galaxy devices (the two most popular smartphones) in the pool. Figure~\ref{fig:m2m_signaling} 
shows that \textit{\ac{IoT} devices generally trigger a higher load on the signaling infrastructure, regardless of the 
infrastructure they use (Diameter or SS7). This holds when checking either the average number of messages per device 
across time as well as the 95\% percentile per hour across all devices. }

% In particular, within the set of clients that buy service from this IPX-P, we identify a specific M2M dataset
%(Table~\ref{table:datasets}) that we analyze further.

\begin{figure}[tbh]
	\centering
	
	\begin{subfigure}{0.95\columnwidth}
		\includegraphics[width=\linewidth]{figures/figs_signaling/mobile_iot_comparison_1109_iphone_m2m_map.png}%
		\caption{\tiny 2G/3G  M2M/IoT devices and smartphone devices.}%
		\label{fig:signaling_m2m_map}%
	\end{subfigure}%
	
	\begin{subfigure}{0.95\columnwidth}
		\includegraphics[width=\linewidth]{figures/figs_signaling/mobile_iot_comparison_1109_iphone_m2m_ngn.png}%
		\caption{\tiny 4G/LTE  M2M/IoT devices and smartphone devices.}%
		\label{fig:signaling_m2m_diameter}%
	\end{subfigure}%	
	
	\caption{\small Signaling traffic statistics for IoT/M2M devices and smartphones. We generate the average per device
		(continuous line) and 95th percentile (shaded area) for each one hour interval over a period of two weeks in November
		2019. }
	\label{fig:m2m_signaling}
	\vspace{-3mm}
\end{figure} 

%\enote{DP}{We should use the same metrics for both this figure and the one in the previous subsection. Also the values
%are quite different and this needs some explanation (unless this is due to different metrics)}


\begin{figure}[tbh]
	\centering
	\begin{subfigure}{0.5\columnwidth}
		\includegraphics[width=\linewidth]{figures/map_roaming_session_length_iot_1109_1121_linkset.png}%
		\caption{\tiny IoT devices.}%
		\label{fig:roaming_session_duration_iot}%
	\end{subfigure}%	
	\begin{subfigure}{0.5\columnwidth}
		\includegraphics[width=\linewidth]{figures/map_roaming_session_length_mobile_1109_1121_linkset.png}%
		\caption{\tiny Smartphones.}%
		\label{fig:roaming_session_duration_smart}%
	\end{subfigure}%	
	\caption{\small Roaming session duration for (a) IoT devices and (b) smartphones.}
	\label{fig:roaming_session_duration}
	\vspace{-3mm}
\end{figure}

We also compare the duration of roaming sessions (i.e., the total number of days a device sent at least one signaling
message while in roaming) for both IoT devices and smatphones. Figure~\ref{fig:roaming_session_duration_iot} show the
number of days an IoT device was active during the two-week period we analyze. We note that the majority of IoT devices 
have long roaming sessions, which in our case cover the entire observation period. This is very different to what we 
observe for smartphones (Figure~\ref{fig:roaming_session_duration_smart}), whose roaming session lengths are shorter. 
This is expected, since \textit{IoT devices are meant to provide services in the country where the IoT provider deploys its services 
during long periods of time, thus becoming "permanent roamers" in the visited country. At the same time, this also translates 
into significant signaling load on the VMNO infrastructure from inbound roaming IoT devices. }

%****************************************

\begin{figure}[h]
	\centering
	\begin{subfigure}{0.5\columnwidth}
		\includegraphics[width=\linewidth]{figures/figs_data/cdf_setup_total_duration.png}%
		\caption{\tiny GTP Tunnel analysis.}%
		\label{fig:GTP_tunnel_stats}%
	\end{subfigure}%	
	\begin{subfigure}{0.5\columnwidth}
		\includegraphics[width=0.95\linewidth]{./figures/figs_data/ip_data_consumption_total_10latam.png}
		\caption{\tiny Data volume per roaming session.}
		\label{fig:roaming_data}
	\end{subfigure}%	
	\caption{\small Analysis of how roamers between countries in Latin America use the IPX-P system: (a)  GTP Tunnel setup delay and total GTP tunnel duration; (b) average amount of traffic roamers generate during their whole roaming session, comparing with IoT devices provisioned by an M2M provider from Spain. }
	\label{fig:data_load_infrastructure}
	\vspace{-3mm}
\end{figure}

\subsection{GTP Tunnels}
Leveraging the data roaming dataset (Table~\ref{table:datasets}) we now characterize the dynamics of the GTP tunnels the IPX-P manages to carry the subscribers' data between the HMNO and the VMNO.
%(see Figure~\ref{fig:data_roaming}, cf. Sec.~\ref{sec:characteristics}).
%The GTP tunnel dynamics have a strong correlation with the load on the IPX-P system to manage them, as well as on the SGSN and GGSN (or PGw and SGw, respectively) that need to maintain the state about these tunnels. 
%Tunnel state is held in the SGSN and GGSN (or PGw and SGw, respectively) as \ac{PDP} Context data structures.
Specifically, we investigate the tunnel setup delay (the time between a PDP Create and its reply) and the total GTP tunnel
duration (the time between a PDP Create and the corresponding PDP Delete event) as they have a strong correlation with the load on the IPX-P, HMNO and VMNO systems.
The tunnel setup delay is an indicator for the amount of processing involved at different network elements for Create PDP messages (as well as the
general processing load). 
A decrease in the average tunnel duration will increase the number of total tunnels and thus also the volume of
signaling messages and the necessary processing for these messages. 
Conversely, longer tunnel duration cause an increased overall memory footprint in the involved nodes to store the PDP
Contexts. 
%After the GGSN/PGw sends the reply for a Create PDP Context, any setup procedures should be completed and the use should
%be able to generate (uplink/downlink) traffic. 
%After the Delete PDP Context, the user traffic is no longer routed.

For the devices roaming within Latin America, we note that, in 80\% of cases, we measure a tunnel setup delay below 1
second (Figure~\ref{fig:GTP_tunnel_stats}).
When verifying the total tunnel duration, we note that on median, the duration of the GTP tunnel is approximately 30
minutes (Figure~\ref{fig:GTP_tunnel_stats}). 
Private conversation with operational teams confirmed us that these values for these metrics are an indication of healthy systems, i.e., processing and storage load at IPX-P, MVNO, HMNO elements are under normal operational conditions.


One likely important factor that influences both these metric is the device type, e.g. phone or IoT \ac{OS}. 
For instance, the \ac{OS} implementation decides when the device should establish a mobile data connection, how long the connection is
held, or which mobile technology takes preference.
%Further, the \ac{OS} transport protocol implementation might impact the tunnel duration properties. 
Since this ecosystem is extremely varied, we are here interested in the aggregated impact on the IPX-P and MNO systems. 
The granular analysis of the device type impact on these metrics is outside the scope of this analysis. 
